Shape Space Spectra

Eigenanalysis of differential operators, such as the Laplace operator or elastic energy Hessian, is typically restricted to a single shape and its discretization, limiting reduced order modeling (ROM). We introduce the first eigenanalysis method for continuously parameterized shape families. Given a parametric shape, our method constructs spatial neural fields that represent eigenfunctions across the entire shape space. It is agnostic to the specific shape representation, requiring only an inside/outside indicator function that depends on shape parameters. Eigenfunctions are computed by minimizing a variational principle over nested spaces with orthogonality constraints. Since eigenvalues may swap dominance at points of multiplicity, we jointly train multiple eigenfunctions while dynamically reordering them based on their eigenvalues at each step. Through causal gradient filtering, this reordering is reflected in backpropagation. Our method enables applications to operate over shape space, providing a single ROM that encapsulates vibration modes for all shapes, including previously unseen ones. Since our eigenanalysis is differentiable with respect to shape parameters, it facilitates eigenfunction-aware shape optimization. We evaluate our approach on shape optimization for sound synthesis and locomotion, as well as reduced-order modeling for elastodynamic simulation.

==> old_background.tex <==
%\section{OLD: A Variational Perspective on Eigenanalysis}





%






%\section{Introduction}

%Eigenfunctions of the Laplace operator are indispensable in a wide array of disciplines, playing a pivotal role in tasks ranging from shape analysis to image processing. However, conventional approaches to compute these eigenfunctions rely heavily on discretized meshes, which often yield results contingent upon the specific mesh used, thus limiting their generalizability and applicability across different domains.

%In this study, we introduce a method for computing eigenfunctions in a continuous manner by leveraging neural fields. Finding the eigenfunctions of the Laplace operator is reformulated according to its variational formulation, which involves minimizing the Dirichlet energy within the domain of our shape of interest, subject to orthogonality constraints with previous eigenfunctions. By sampling the domain and using the gradient of the neural field, we can calculate the Dirichlet energy and formulate an appropriate loss function that minimizes this energy. The orthogonality constraints are satisfied by following the Gram–Schmidt process, which "projects out" previous eigenfunctions. It can be proved, and is shown experimentally, that minimizing the Dirichlet energy inherently satisfies the vanishing Neumann boundary conditions. 

%Thus, the straightforward approach to calculating continuous eigenfunctions using neural fields involves first finding a function that minimizes the Dirichlet energy within the shape of interest and is orthogonal to the constant function. Once the first eigenfunction is trained, the second eigenfunction is found by ensuring orthogonality to both the first eigenfunction and the constant function, while also minimizing the Dirichlet energy. This process is repeated to obtain subsequent eigenfunctions. Let's call it the sequential process.


%The aforementioned sequential process process systematically identifies the 1st, 2nd, 3rd, and subsequent eigenfunctions, each corresponding to the minimal, second-minimal, third-minimal, and so forth, Dirichlet energy. This method works well for a single shape. But how do we extend this to train across different shapes? We might want to add some shape information (e.g., a geometry code) and apply the same process to different shapes. First, we find the eigenfunction with the minimal Dirichlet energy across the training set, then the second one by projecting out the first, and so on. However, this approach can be problematic.

%Consider the scenario where the geometry code $\bm{g}$ encodes the width of a rectangular shape while keeping the length fixed. As shown in in Figure \ref{fig:compare_sort}. As the width increases, the predicted eigenfunction changes accordingly:
%\begin{enumerate}
%    \item When the width is smaller than the length, the second eigenfunction (first non-constant eigenfunction) is a sinusoidal function along the vertical direction.
%    \item When the width equals the length, symmetry allows multiple eigenfunctions.
%    \item As the width grows larger than the length, the second eigenfunction shifts to a sinusoidal pattern along the horizontal direction.
%\end{enumerate}
%This "sudden change" is illustrated in the left part of Figure \ref{fig:compare_sort}, where the green line (eigenvalue for the first non-constant eigenfunction) remains constant initially and then decreases as the width becomes dominant, while the red line (eigenvalue for the second non-constant eigenfunction) follows a similar pattern. As a result, using the Gram–Schmidt process with a fixed order will result in finding functions that follow the green and red eigenvalues shown on the left. Is that really what we want? Instead, by allowing crossovers between shapes, as shown on the right side of Figure \ref{fig:compare_sort}, we can encourage the neural networks to learn smoother eigenfunctions that span the same space as the left eigenfunctions.

%So how do we allow crossovers? The reason the previous sequential process enforces a non-crossover pattern is that it assigns a fixed order to each learned function. When learning the first function, if we achieve perfect optimization, it must be the function with the minimal Dirichlet energy subject to one orthogonal constraint (to the constant function) for all the shapes within the training set. We can allow crossovers by reordering the functions of interest. To achieve this, we:
%\begin{enumerate}
%    \item Train the top $k$ eigenfunctions simultaneously instead of one at a time.
%    \item Dynamically reorder the eigenfunctions during each training epoch so that the orthogonal constraints differ for different shapes.
%\end{enumerate}

%Our method presents several distinct advantages. Notably, it enables learning across families of shapes, facilitating applications such as the prediction of eigenfunctions on incomplete shapes and enabling interactive manipulation across shape families. We show that our dynamic reordering encourages smoother eigenfunctions across different shapes. Furthermore, our approach transcends the limitations of traditional discrete operators by extending to higher dimensions, where discrete methods are less explored, opening up new avenues for exploration and application.


% Head 1
